PATIENT-{\Psi}: Using Large Language Models to Simulate Patients for Training Mental Health Professionals

Mental illness remains one of the most critical public health issues. Despite its importance, many mental health professionals highlight a disconnect between their training and actual real-world patient practice. To help bridge this gap, we propose PATIENT-{\Psi}, a novel patient simulation framework for cognitive behavior therapy (CBT) training. To build PATIENT-{\Psi}, we construct diverse patient cognitive models based on CBT principles and use large language models (LLMs) programmed with these cognitive models to act as a simulated therapy patient. We propose an interactive training scheme, PATIENT-{\Psi}-TRAINER, for mental health trainees to practice a key skill in CBT -- formulating the cognitive model of the patient -- through role-playing a therapy session with PATIENT-{\Psi}. To evaluate PATIENT-{\Psi}, we conducted a comprehensive user study of 13 mental health trainees and 20 experts. The results demonstrate that practice using PATIENT-{\Psi}-TRAINER enhances the perceived skill acquisition and confidence of the trainees beyond existing forms of training such as textbooks, videos, and role-play with non-patients. Based on the experts' perceptions, PATIENT-{\Psi} is perceived to be closer to real patient interactions than GPT-4, and PATIENT-{\Psi}-TRAINER holds strong promise to improve trainee competencies. Our code and data are released at \url{https://github.com/ruiyiw/patient-psi}.

==> sections/alt_intro.tex <==
\section{Condensed Introduction}
\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{figs/cog_model.pdf}
\caption{The illustration of our idea.} 
\label{fig:cog_model}
\end{figure}
The gap between available mental health support and patient needs is a critical issue, with one in eight people globally living with mental health conditions (World Health Organization, 2023) despite every 6 in 10 psychologists no longer having openings for new patients.
Training mental health professionals requires extensive effort, yet many professionals highlight a disconnect between their training and the complexities of real patient interactions. 
To understand these training challenges, we conducted a formative study involving semi-structured interviews with twelve domain experts --- including current Master's of Social Work students, licensed social workers, and clinical psychologists. 
This diverse group provided insights into the difficulties faced when transitioning from formal CBT training to real-world practice (more details in~\Cref{appx:formative_study}).
All experts noted that their training did not adequately prepare them for the unpredictable and multifaceted nature of real patient interactions.
Despite wanting more interactive experiences, experts found role-playing exercises with their peers based on manuals, a common training method, to be unrealistic, as these exercises often do not reflect the nature of actual therapy sessions. 


Building on these insights, we propose using large language models (LLMs) to create high-fidelity simulated therapy patients as a means of improving the realism and effectiveness of mental health training. 
There has been growing interest on developing LLM-based methods for psychology~\citep{chen2023empowering} due to their promising performance in basic theory of mind capabilities~\citep{bubeck2023sparks,kosinski2023theory}. \ruiyi{[comment: I think mentioning the term \textit{theroy of mind} in the intro might cause reviewers to think critically about our paper - may be consider mentioning \textit{LLM therapists, LLM as clinical agents, agent-based hospital simulations, etc.}]}
Our goal is to leverage these capabilities to develop a training tool that bridges the gap between existing training methods and the complexities of real patient interactions.

We introduce \patient, a novel simulated patient agent that integrates cognitive modeling with LLMs. 
\patient incorporates diverse patient cognitive models based on CBT principles. 
We collaborate with clinical psychologists to curate a set of high-quality, diverse patient cognitive models by asking them to annotate LLM-generated cognitive models. 
We additionally incorporate six conversation styles identified through our formative study, enabling \patient to more closely mimic the complex dynamics of real patient communications.

To enable training with \patient, we propose \trainer, an interactive training framework where trainees practice CBT cognitive model formulation using \patient. 
Trainees engage in conversations with \patient to develop its cognitive model, then compare their results with the reference model used to program \patient. 
This feedback mechanism is designed to improve skills in CBT formulation, directly addressing the key challenges identified in our formative study.

To validate our approach, we conducted a user study with $15$ mental health trainees and $20$ experts. 
The study demonstrated that \patient closely resembles real patients in terms of symptoms, cognitions, communication styles, and emotional states, outperforming GPT-4. 
Experts reported significant perceived improvements in CBT formulation skills when practicing with \trainer, noting that it better prepares trainees for real patient interactions. 
Additionally, \trainer offers several advantages over traditional training methods, such as customizable patient interactions and a safer training environment. \textcolor{red}{TODO: update with new results}

Our contributions are summarized as follows:
\begin{contributionenum}
\item Based on our interviews with mental health domain experts, we propose \patient, the first integration of CBT cognitive models with LLMs to simulate patients with mental health disorders.
\item We introduce \trainer, an interactive training framework using \patient for trainees to practice CBT formulation skills.
\item We create and release dataset consisting of 118 CBT cognitive models generated by GPT-4-Turbo and refined by clinical psychologists.
\item Our user study with both mental health trainees and experts demonstrates that \patient exhibits high fidelity to real patients, and practicing with \trainer significantly improves perceived skills and confidence in CBT formulation.
\end{contributionenum}


==> sections/formative.tex <==
\section{Formative Study}
We first conducted a formative study in the form of semi-structured interviews with domain experts. %to understand challenges and elicit feedback on a prototype of \trainer. 
%In our formative study, we conducted semi-structured interviews with individuals with varying levels of CBT training and real patient experience. 
%two distinct groups to inform the development of our framework.
%The first group consisted of individuals who have studied CBT but have not yet practiced it with real patients. 
%In engaging with this population, our goal was to understand the challenges encountered in the CBT training process and how our framework could be situated with these challenges.
%We also sought to understand their impression of the simulated patient framework in the context of their current studies or patient experience.
We interviewed twelve individuals who had diverse educational backgrounds and career experiences. 
Among them, five were Master's students, while the rest included a Ph.D. student, a post-doctoral fellow, three licensed social workers, and two psychologists.  
Our participants also had varied levels of experience working with patients.
Only one individual had not yet worked with any patients, while another reported working with anywhere from 1500-3000 patients over their career. 
%The students we interviewed most commonly mentioned working with 10-40 patients in various capacities, such as CBT group sessions or one-on-one counseling.
We refer to individuals as \textit{experts} if they received a graduate degree and have worked with at least 5 patients; we use \textit{trainees} if they do not have a graduate degree and have formal experience with fewer than 5 patients. 
In our interviews, we first asked the experts questions about challenges they faced transitioning from their formal CBT training to practice. % their experiences during their CBT training, working with real patients, or the transition period.
We then presented both groups with a prototype of \trainer to elicit feedback.
%The second group included individuals who have both studied CBT and applied it in real-world scenarios with patients.
%With this group, our goal was to capture the difficulties in transitioning from theory to practice. 
%We also sought to understand their impressions of using simulated patients to improve the realism and utility of the framework. 



%\subsubsection{General Feedback}
\paragraph{Challenges}
%The experts identified several challenges when transitioning from formal training to practice. 
100\% of experts noted that their training did not adequately prepare them for the complexities of real-world practice,
where patients often experience co-occuring challenges, such as other mental health issues or poverty. 
%One expert highlighted, ``The biggest difference ... was when you are in training ... it's usually [that] the prototype or the example person has one diagnosis. It's very clean cut.'' 
Experts found role-playing exercises with their peers based on manuals to be unrealistic, as these exercises often do not reflect the unpredictable nature of actual sessions. 
One participant explained, 
\begin{formal}
   Manuals can often make it feel quite clean. But then when you're in the room with the patient, what they're actually saying can feel very messy. 
\end{formal} 
\noindent This gap made it difficult for some experts to develop confidence in their skills: the examples were too perfect to apply in practice. 
%To address this gap, many participants suggested incorporating more realistic and varied examples during training to help trainees practice critical clinical skills, such as handling patient pushback or maintaining therapeutic dialogue.
%Taken together, these findings indicate a need for more diverse and realistic training scenarios that allow trainees to practice critical clinical skills.%, like maintaining dialogue and handling the complexities of real patients.


\paragraph{Fidelity}
To address this gap, many participants suggested incorporating higher fidelity and varied examples during training to help trainees practice critical clinical skills. %, such as handling patient pushback or maintaining therapeutic dialogue. 
When asked to provide feedback on the prototype, five of the seven experts emphasized the importance of fidelity in the simulated patient interactions and representations.\footnote{Two experts provided low-level commentary on practical design choices, so their input with respect to fidelity is not available.}
Six of the seven experts noted the importance of including diverse patient types to mirror those encountered in practice. 
%These include patients with different levels of support and access to resources, as well as those facing different challenges. 
%Additionally, the experts noted that the situations encountered by participants would also likely be reflected in the other dimensions. For example, someone without a social support network may primarily remark on interpersonal relationships with a landlord or doctor, rather than family. 
They further identified dimensions along which patients could vary, which may contribute to their level of difficulty for a new clinician. 
They highlighted that more difficult patients might be more oppositional, express themselves more verbosely in a way that may not answer the questions, provide less information and be guarded, or go off on tangents. 
Another expert mentioned that some patients may be more of ``people pleasers'', making them more likely to tell the therapist what they want to hear, rather than sharing what is happening in their lives. 
One expert emphasized, 
\begin{formal}
    People probably aren't going to fit neatly into the modality. And that's okay. That's just something to be prepared for.
\end{formal} 
\noindent These findings indicate the need for a training framework with extensive customization: patients should have varied experiences and emotional responses. % that are relatively consistent with other factors in their lives.


\paragraph{Effectiveness}
We also discussed the effectiveness of an AI-powered patient simulation tool for CBT training. 
All experts were positive about the possibility for trainees to receive AI-powered training using the tool. 
In particular, they saw benefit in the customization options afforded by AI and connected it to our discussions about trainee challenges by noting its ability to let students to try different diagnoses, different comorbidities, and diverse backgrounds or conversational styles. 
The experts also highlighted that a well-designed simulation could improve training over role-playing based on manuals: the presence of a transcript would enable the instructor to provide real-time or post-hoc feedback. 
The trainee who had not yet used CBT with real patients remarked that they believed the tool would make them feel more confident navigating future conversations with real patients. 
These findings indicate that this tool could help address some of the existing challenges through its customization, flexibility, and ability to incorporate feedback.

%\subsubsection{Non-Student Feedback}


==> sections/method.tex <==
\section{Methodology}
In this section, we will first introduce the cognitive modeling schema in CBT, which we use to build \patient. Then we will elaborate our proposed simulated patient, \patient (\S\ref{method_patient}), and the training framework \trainer (\S\ref{method_trainer}). Figure~\ref{fig:overview} illustrates the overview of our method.

\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{figs/overview.pdf}
\caption{The overall framework of \patient and \trainer.} 
\label{fig:overview}
\end{figure*}

\subsection{Cognitive Modeling in CBT}
\label{method_cbt}
%goal of this section: what this is, justify why we do it this way. Jamie to take a pass at editing.
In CBT~\cite{beck2020cognitive,hollon2013cognitive,hofmann2012efficacy}, formulating and constructing a patient's cognitive model is a crucial stage through therapeutic conversations. Such cognitive model, named Cognitive Conceptualization Diagram (CCD), systematically represents the network of a patient's \textit{core beliefs}, \textit{intermediate beliefs}, \textit{intermediate beliefs during depression},
\textit{coping strategies}, as well as the triggering \textit{situations}, \textit{automatic thoughts}, \textit{emotions}, and \textit{behaviors}. Figure~\ref{fig:ccd} shows an example CCD in flat format. 

\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{figs/CCD_example.png}
\caption{An example cognitive model (CCD) in CBT.} 
\label{fig:ccd}
\end{figure}


Core beliefs are the deeply ingrained, fundamental perceptions individuals have about themselves, others, and the world. People with mental health disorders typically hold unhealthy core beliefs, such as \textit{I'm unlovable}, \textit{I'm a failure}, etc. 
Intermediate beliefs, which include rules, attitudes, and assumptions, stem from these core beliefs and influence a person's thought patterns, e.g., \textit{If I cannot meet the expectations of others, then I'm a failure}.
Coping strategies are the behaviors and thoughts developed over time to manage distress, such as \textit{avoidance}, \textit{emotional numbing}, etc. The CCD links these cognitive elements to specific situations, highlighting how they trigger automatic thoughts, emotions, and behaviors. For example, a situation may activate an automatic thought rooted in a core belief, leading to emotional responses and behaviors. By modeling these underlying cognitive structures, CBT practitioners can better develop targeted interventions to modify maladaptive beliefs and promote healthier cognitive and behavioral patterns. In this work, we use the CCD as the cognitive model to integrate with an LLM to simulate a patient communicating in a way matching the underlying CCD. 


\subsection{\patient}
\label{method_patient}
% Define terms: cognitive models 
\paragraph{Cognitive Models Creation}
% Why creating? There is no existing work providing the complete cognitive models in NLP research; text-book examples are limited and not diverse enough to represent a wide range of patients
% According to \citet{beck2020cognitive}, a patient's cognitive model (CCD) includes \textit{situation}, \textit{emotions}, \textit{behaviors}, \textit{automatic thoughts}, \textit{intermediate beliefs}, \textit{core beliefs}, and \textit{coping strategies}. 
To the best of our knowledge, no existing work offers a dataset of CCDs due to the data privacy constraints involved in acquiring real patient data, as well as the high-level expertise required to do manual compositions or annotations. 
In this work, we create cognitive models combining GPT-4 data synthesis and revisions by domain experts. 

\begin{table*}[t]
\centering
\begin{tabular}{>{\ttfamily}l p{13cm}}%p{6cm}}
\toprule
\textnormal{Relational Style} & Description \\
\midrule
plain & Direct and straightforward communication. A simpler relational style for practice. \\
upset & Expresses frustration. May exhibit resistance toward the therapist or process. \\
verbose & Uses more words than necessary. Therapists may find it hard to guide the conversation.  \\
reserved & Minimal and restrained communication. \\
tangent & Deviates from the main topic. May demonstrate reluctance to share or express distrust.  \\
pleasing & Attempts to be agreeable without fully understanding or agreeing. \\
\bottomrule
\end{tabular}
\caption{Different relational styles that \patient can take on, with descriptions. }
\label{tab:relational_styles}
\end{table*}

To obtain diverse cognitive models that match real patients, we take the real therapy session transcripts obtained from the collections of the ``Counseling and Therapy'' subject with the keyword ``Cognitive Behavioral Therapy'' in the publically available Alexander Street database\footnote{\url{https://alexanderstreet.com/}}. We prompt GPT-4-Turbo with the transcripts and a one-shot example of a full cognitive model obtained from a textbook~\citep{beck2020cognitive}. Then, two clinical psychologists %(our co-authors) 
manually modified the LLM-derived cognitive models, resulting in an expert-verified dataset containing 118 cognitive models paired with relevant patient histories, each with one activating situation. 
Note that formulating the full cognitive model with multiple activating situations of a patient could be a very long process spanning multiple sessions. In this work, we start with the sub-process of formulating a partial cognitive model from a single activating situation, which is typically conducted within one session.
% The detailed data collection procedure, prompts for generating cognitive models, and expert validation protocol are detailed in Appendix \S\ref{app:cog_gen}. 
%\textcolor{green}{maybe just say modification / what you have said before? can also just say ``The entire protocol is detailed in Appx blahblah'' to avoid giving a specific name}

\paragraph{Patient Simulation} The interplay between thoughts, feelings, and behaviors, as well as the deep connections with layers of beliefs described by a cognitive model, are essential for replicating a real patient's communicative behaviors. 
Besides the cognitive model, real patients also have different relational styles during the therapeutic conversation with the therapists. Based on consultations with domain experts in our formative study, we included six relational styles that our simulated patient, \patient can take on: 
\texttt{plain}, \texttt{upset}, \texttt{verbose}, \texttt{reserved}, \texttt{tangent}, and \texttt{pleasing}. 
\Cref{tab:relational_styles} provides a description of each of these styles.

Domain experts (our co-authors) further annotate each patient's cognitive model with a list of valid relational styles and develop instructions for the LLM to follow in order to simulate a patient for each style.
Then, we prompt GPT-4 to build \patient, consisting of the relational style prompt, the patient cognitive model with the relevant history, and a list of instruction prompts focusing on authenticity and consistency of the simulated patient communicative behaviors. The model is then continually prompted to engage in a CBT-based therapy session role-playing a patient with the corresponding cognitive model and relational styles. 
% The prompts for the patient agents are provided in Appendix \S\ref{app:prompt}.


\subsection{\trainer}
With \patient, we propose \trainer, an interactive training framework for mental health professionals to practice cognitive model formulation in CBT. \trainer enables interactive training through three steps: 1) interacting with \patient for a CBT session, 2) formulating the cognitive model of \patient, and 3) reviewing the original cognitive model used to build \patient as a reference to get feedback. See Figure~\ref{fig:overview} for an illustration of the training procedure.

We build a web application for \trainer that presents \patient on a chat interface and implements the interactive training framework. First, \trainer provides the option of choosing a patient with different relational styles. Then, a trainee initiates the therapy session with \patient after reviewing the provided patient's relevant history. During the session, the trainee is tasked with formulating the cognitive model of \patient from their conversation.
After concluding the therapy session, the trainee compares the formulated cognitive model with the original cognitive model used to program \patient. 
This comparison enables the trainee to obtain real-time feedback on their CCD formulation accuracy. We present screenshots of the interface of \trainer in Appendix \S\ref{app:inter}.
% Learning through interaction and comparison enables the trainee to gain CBT skills and confidence of interacting with real patients in the future. 

\label{method_trainer}


==> sections/user_study.tex <==
\section{Experimental Setup}
In this section, we present the experimental results evaluating the efficacy of \trainer, our patient simulation framework.
%Our user study is designed to answer the following research questions:

\paragraph{Baseline} We compared \trainer with a baseline of vanilla GPT-4. 
In the GPT-4 baseline, instead of the curated cognitive models, we only use a general description of patients with depression or anxiety as the input to the LLM. 
Therefore, we cannot incorporate the feedback mechanism and show the reference cognitive model to the trainees in the baseline. 
The baseline also does not include customized options for different patient types.

\paragraph{Recruiting Mental Health Experts and Trainees}
We recruit both mental health experts in CBT and trainees (students) to understand both perceptions of the tool -- from those with years of real patient experiences (experts), as well as those who would mostly be using it (trainees). 
The recruitment is conducted through the professional networks of our co-authors in mental health (professors and Ph.D. students in clinical psychology and social work). 
We also used snowball sampling.
For recruitment, we defined experts as those with a graduate degree in clinical psychology, social work, or other related majors and have worked with at least 5 patients.
We defined trainees as those still in school/training with fewer than 5 real patient experiences.
%We pay a \$60 Amazon gift card to each participant. 
%Our study is IRB approved; s
See \S\ref{ethics} for more details about the recruitment procedure. 
We present our results for 14 participants --- 10 experts and 4 trainees --- in this preliminary version. 

\paragraph{Study Protocol}
The study was conducted over Zoom.
Participants were asked to interact with both versions of the tool and provide feedback through a structured survey, which contained specific questions tailored to each group.
All participants were asked to think aloud while interacting with the tool, and we encouraged them to verbally answer the free-form survey questions to elicit more detailed answers.
To control for ordering effects, we randomized the order in which the participants interacted with both tools.
All participants practice for two sessions. We instructed the experts to practice with two patients with different relational types. 
Trainees are asked to choose the types based on their own level and confidence, so they may practice with the same type. %since they mostly have limited real patient experiences, we instruct them to choose two types based on their own level and confidence. 
However, we ensured that the patients had different underlying cognitive models to maximize coverage of our curated cognitive models.  
For a more detailed analysis of the study data, please see \Cref{sec:user_study_design_details}.

\begin{comment}
\noindent \textbf{Metrics}
\textcolor{green}{considering cutting and placing in the appropriate sections, since it might be annoying to continuously refer back to this. also might be better to use this space to say more about the questions/what we are eval?}
We asked the participants two types of questions: pairwise comparisons and individual assessments, both using a 5-point Likert scale. 
%For both types of questions, we used a 5-point Likert scale.
For the pairwise comparison questions, the scale indicates degrees of preference: higher means more preference for \patient or \trainer. 
Lower means more preference for the baseline. 
%$1$: the baseline is much better, $2$: the baseline is somewhat better, $3$: the two are about the same, $4$: our tool is somewhat better, and $5$: our tool is much better.
%For these questions, that means that values closer to $5$ indicates a stronger preference for our tool. 
For individual assessments, the $5$-point scale corresponds to level of agreement with a statement about one of the two variants, ranging from strongly disagree (1) to strongly agree (5). %($1$: strongly disagree, $2$: somewhat disagree, $3$: neither agree nor disagree, $4$: somewhat agree, and $5$: strongly agree).
\end{comment}

\section{Expert Evaluations}
Experts evaluated both the resemblance of the \patient with real patients (fidelity) and the potential for improving CBT training of \trainer(effectiveness), since they have rich experiences in real patient interactions.
%In our analysis of the expert comparisons, we conducted a one-sided Wilcoxon signed-rank tests for all pairwise comparisons to discern whether \patient was more preferred to the baseline.
%To account for multiple comparisons and control the family-wise error rate, we then applied the Holm-Bonferroni correction to the p-values obtained from these tests. 

\subsection{Fidelity of \patient} 
Experts provided pairwise comparisons of \patient and the baseline-generated patients on a $5$-point Likert scale to evaluate their fidelity compared to real patients. 
Higher values indicated a preference for \patient. 
Across all dimensions, \patient is perceived as more closely resembling real patients, outperforming GPT-4.

Not only did experts find the interaction experience with the patients to be more realistic (median: $4.5$, IQR: $4.0$-$5.0$), they also largely agreed that \patient{} was more similar to real patients (median: $4.0$, IQR: $3.0$-$5.0$).
We asked the experts to further evaluate the two according to specific, important factors for creating a cognitive model (CCD): the exhibited symptoms and expressed cognitive model, emotional states, and relational styles. 
Compared to the baseline, \patient{} was rated higher along all factors: it better represented the symptoms and cognitive models (median: $4.0$, IQR: $3.0$-$5.0$), the emotional states (median: $4.0$, IQR: $3.5$-$5.0$), and the relational styles (median: $4.0$, IQR: $4.0$-$5.0$) of real patients. 

%When comparing the overall resemblance to real patients, $7$ of $10$ experts agreed that \patient{} was somewhat better to much better at resembling real patients (median: $4.0$, IQR: $3.0$-$5.0$).
%Experts also mentioned that the experience of interacting with the patient through \trainer was more realistic (median: $4.5$, IQR: $4.0$-$5.0$). 

\begin{comment}
The statistical analysis further confirmed these observations, showing significant differences along all comparisons at a significance level of $\alpha=0.05$.
Indeed, \patient was assessed as significantly better at resembling real patients (Wilcoxon statistic: $33.5$, $p=0.013$).
It was also assessed as significantly better at representing the symptoms and cognitive models (Wilcoxon statistic: $15.0$, $p=0.019$), the emotional states (Wilcoxon statistic: $36.0$, $p=0.005$), and the communication styles (Wilcoxon statistic: $45.0$, $p=0.003$).
\trainer was also assessed as providing higher-fidelity experiences of interacting with real patients (Wilcoxon statistic: $52.5$, $p=0.004$). 
This demonstrates that \patient provides higher-fidelity simulations of real patient interactions, emotional states, communication styles, and cognitive models. 
%\textbf{something that would add to the analysis: can we say something about the factors that those who said they were the same were attending to? for example, if these people focused on things like lack of verbal communication, their feedback is less useful than someone who was actually comparing the two tools against each other (rather than just saying that overall text interactions are not that realistic)}
\end{comment} 

\patient was perceived as providing a more realistic challenge of extracting detailed information from patients, whereas the baseline was perceived as being too forthcoming with its responses.
This ease of extracting information was perceived as unrealistic because it indicated a level of clinical insight into one's own experiences that a patient seldom has. 
One expert %, who had experience with over 120 patients, 
noted that the nature of the baseline responses %was more characteristic of a therapist than a patient, stating it 
``was almost like doing therapy with a therapist.'' This is likely because GPT-4 is pre-trained on an extensive corpus of therapy knowledge and merely applies that knowledge in a therapeutic setting. This underscores the challenges of simulating the communicative behaviors of real patients with mental health disorders, even with the most advanced LLM.
Taken together, \patient{} is assessed as having higher fidelity in representing real patient characteristics.

\begin{comment}
Experts generally agreed that there were certain aspects of the baseline patient that did not align with their real patient experiences.
Specifically, it was perceived as being too forthcoming with its responses, indicating a level of clinical insight into their own experiences that patients seldom have.
One expert, who had experience with over $120$ patient, noted that the nature of the responses was more characteristic of a therapist than a patient, stating it ``was almost like doing therapy with a therapist.''
In contrast, \patient{} was perceived as more realistic, especially in terms of the difficulty in extracting detailed information from vague statements. 
This difference was highlighted in the context of the \texttt{Tangent} patient type, where \patient{} allowed trainees to practice refocusing efforts in a way that judged to be more aligned with real-life scenarios.
Participants found the tangents provided by the baseline \texttt{Tangent} patient to be too structured. 
\end{comment}

\subsection{Effectiveness of \trainer}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/user_study_data_analysis_prelim/expert_trainee_skills.png}
    \caption{Score distribution for expert comparison of the effectiveness of the baseline and \trainer for improving trainee skills. 
    The y-axis represents the score, ranging from 1 (the baseline is much better) to 5 (\trainer is much better). 
    }
    \label{fig:skill_improvement_results}
\end{figure}
Evaluating the perceived effectiveness of training tools is crucial to ensure they provide meaningful and realistic learning experiences for trainees.
To evaluate this, experts provided pairwise comparisons of \trainer{} and the baseline framework on a $5$-point Likert scale.
Again, higher values indicated a preference for \trainer. 
%found \trainer{} to be more useful than the baseline for improving overall skills in CBT diagnosis training.
%On a 5-point Likert scale with associated labels, shown in~\Cref{fig:skill_improvement_results}, 
\Cref{fig:skill_improvement_results} shows the results.
Experts believed \trainer{} would be more effective than the baseline at improving overall CBT skills (median: $4.5$, IQR: $4.0$–$5.0$). %, indicating that the experts believed it would be more effective than the baseline at improving overall CBT skills.
Specifically, experts believed \trainer{} would be more effective at helping trainees identify beliefs (median: $5.0$, IQR: $3.0$–$5.0$) and maladaptive thinking (median: $5.0$, IQR: $4.0$–$5.0$). 
%Importantly, experts indicated that \trainer{} would provide somewhat to much better realistic experiences of interacting with patients (median: $4.5$, IQR: $4.0$–$5.0$).

We then asked experts to compare \trainer to existing CBT training techniques.
Experts indicated that \trainer would be more effective than these techniques at improving overall CBT formulation skills (median: $5.0$, IQR: $4.0$-$5.0$), including helping trainees identify beliefs (median: $5.0$, IQR: $4.0$-$5.0$) and maladaptive thinking (median: $5.0$, IQR: $4.0$-$5.0$).
We then investigated what factors contributed to this assessment.
$90$\% of experts indicated that \trainer was more easily accessible than existing techniques, while $100$\% of experts preferred its customization options to practice with different patients. 
$50$\% of experts appreciated the first-hand, interactive experiences that it afforded.
Taken together, these results indicate that \trainer offers many practical benefits that contribute to its perceived efficacy at improving CBT formulation skills compared to both a strong GPT-4 baseline and current training tools.

\begin{comment}
These results showed significant differences $(\alpha=0.05)$.
Indeed, \trainer was assessed as significantly better than the baseline for its potential to improve over skills (Wilcoxon statistic: $45.0$, $p=0.003$).
It was also assessed as significantly better at helping trainees identify beliefs (Wilcoxon statistic: $28.0$, $p=0.006$) and maladaptive thinking (Wilcoxon statistic: $36.0$, $p=0.004$).
This demonstrates that the patients provided by \trainer are perceived as more useful for preparing trainees. 
\end{comment}

\paragraph{Use in Practice}
Given the perceived effectiveness of training tools, evaluating the likelihood of experts adopting these tools in practice is crucial to ensure their potential impact translates into real-world settings. 
When asked which of the two options was better for CBT training, experts overwhelmingly preferred \trainer{} (median: $5.0$, IQR: $4.0$–$5.0$). 
We also asked the experts to indicate which of the two options they would be more likely to use as a training tool.
A majority (8 out of 10) preferred \trainer{} for use in their classrooms and training programs (median: $5.0$, IQR: $4.0$–$5.0$). 
The remaining 2 experts were equally likely to use either option, and no experts preferred the baseline.
%\textbf{mention stat analysis. overall better: Wilcoxon statistic: 43.0; P-value: 0.005930764660659649. likelihood to use: Wilcoxon statistic: 36.0; P-value: 0.00414960799764038}

\paragraph{Effectiveness of Individual Components}
\begin{comment}
Here we present the results from asking the experts to individually assess the tools by indicating their level agreement with the provided statements.
For this set of results, $1$ indicates strong disagreement, $3$ indicates indifference, and $5$ indicates strong agreement.
We ask participants these questions to understand how each variant compares with the current training materials, such as role plays and textbook examples. 
One interesting finding is that, similar to our findings in the formative study, experts were generally optimistic about the utility of AI-powered training tools. 
Experts indicated agreement that both the baseline and \trainer could provide more realistic experiences in comparison to current materials (respectively, median: $4.0$, IQR: $3.0$-$5.0$; median: $4.0$, IQR: $4.0$-$5.0$); however, there was more consensus that \trainer could provide a more realistic experience. 
When asked which features contributed to the benefit of the tool, 100\% of experts attributed customization options as a benefit of \trainer, compared to only 30\% of experts for the baseline. 50\% of experts appreciated the diverse patient profile types of \trainer, compared to 30\% of experts for the baseline.
90\% of experts viewed the ease of access as a benefit of AI-powered training tools more generally.
\textbf{prob fix above to just talk about specific features of our tool, comparison may be confusing }
\end{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/user_study_data_analysis_prelim/expert_assessment_components.png}
    \caption{Expert preferences for two key contributions of \trainer: building simulated patients based on a reference CCD, such that it can be displayed to provide feedback, and engendering the ability to practice with different types of patients.}
    \label{fig:results_indiv_components}
\end{figure}
%\textcolor{green}{maybe fold into previous so that all effectiveness is together}
Following the strong preference for \trainer, we present the results from expert’s individual assessment of the key components of our method: the ability to display an accurate reference cognitive model (CCD) and the ability to practice with diverse patient relational types. 
Experts rated their agreement with specific statements on a scale from 1 (strong disagreement) to 5 (strong agreement). 
\Cref{fig:results_indiv_components} shows our main results. 
100\% of experts preferred that \trainer display the reference CCD. %, with 5 somewhat agreeing and 5 strongly agreeing. 
%100\% of experts also 
and preferred the option to practice with patients of different relational types over not. 
These findings indicate that experts highly value \trainer’s features of showing a reference CCD and offering diverse patient types, both of which are viewed as crucial for effective and realistic training.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/user_study_data_analysis_prelim/accuracy.png}
    \caption{Perceived accuracy of \trainer in representing the various components of the reference cognitive model (CCD). According to experts, nearly 80\% of the patients were very to extremely accurate overall.}
    \label{fig:results_accuracy}
\end{figure}
\paragraph{Perceived Accuracy} Finally, we further investigate the practical utility and effectiveness of \trainer by asking the experts to assess the accuracy of the simulated patients across all of the dimensions included in the CCD. 
\Cref{fig:results_accuracy} shows the results of this assessment. 
The results indicated a high level of accuracy across all dimensions: 75\% of the simulated patients were rated as being very to extremely accurate overall. 
In fact, 75-90\% of the simulated patients were evaluated as being very to extremely accurate across all of the specific dimensions. 
These findings suggest that \trainer provides a reliable tool for students to practice and verify their understanding against accurate simulated patient behaviors.

\begin{comment}
\paragraph{Effectiveness of Showing Cognitive Model}
A crucial component of \trainer is that each patient is associated with a specific reference CCD. 
This feature enables us to show this reference CCD to allow trainees to obtain feedback on their own CCD construction. 
$100$\% of experts agreed that they not only preferred that \trainer{} show the reference CCD over not showing it (5 somewhat agree, 5 strongly agree), but they also believed that seeing the reference CCD is useful for practicing skills (3 somewhat agree, 7 strongly agree). 
These results are further supported by our findings that experts found the \patient to overall accurately reflect the reference CCD (median: $4.0$, IQR: $3.5$-$4.5$).

\paragraph{Effectiveness of Patient Types}
Another critical feature of \trainer is the ability of trainees to practice with diverse patient types to better prepare trainees for the intricacies of real-patient interactions.
$90$\% of experts agreed that the option to practice with different patient types is useful for preparing for real-patient interactions (3 somewhat agree, 6 strongly agree). 
Furthermore, $100$\% of experts agreed that they preferred the option to practice with different patients over not (7 strongly agree, 3 somewhat agree). 
\end{comment}

\begin{comment}
\subsubsection{Feedback and Discussions}
[not totally sure what to put here based on the summaries]
We also asked the experts to suggest improvements for the tool overall.
One participant suggested that incorporating more descriptive prompts for different cognitive conceptualization fields would be helpful to remind trainees of the differences between the more technical jargon (e.g., the difference between core belief and intermediate belief).
Another participant expressed a desire for the inclusion of ``talking" avatars to move toward even more realistic interactions. 
Experts generally were in favor of the simulated patients being less generous with information, as it would provide more challenging and accurate clients for the trainees to practice with. 
Experts also commented on details like the timing of patient responses: one expert mentioned that typical patients would not respond as quickly as the simulated patient. 
In the future, this timing aspect could be customized to support the emotional states of the patients. 
For example, a patient experiencing depression could respond more slowly to reflect symptoms like slower reaction times, difficulty concentrating, or general fatigue.
\end{comment}

\section{Trainee Evaluations}
Trainees compared the tool along three key dimensions: perceived practical utility, perceived skill improvement in CBT, and perceived confidence improvement for real patient interactions.

\paragraph{Perceived Practical Utility}
To evaluate the perceived practical utility, we asked the trainees to indicate their overall preferences and likelihood of use in practice.
Trainees compared \patient and the baseline on a $5$-point Likert scale, in which higher values indicate a higher preference for \trainer.
Both trainees indicated that they preferred \trainer{} overall for CBT training, with a median score of $4.5$ (IQR: $3.5$-$5.0$). 
Trainees also indicated that they were more likely to use \trainer{} in practice, with a median score of $3.5$ (IQR: $3.0$-$4.5$).
These findings highlight that trainees and experts are similar in their likelihood of practical adoption of \trainer.
%Interestingly, the participant that rated the two variants more similarly was the trainee without real patient experience. 
%When asked to compare the realism for real patient interactions, this participant rated the baseline as being somewhat better, contradicting the evidence provided by the experts that \trainer{} more accurately resembles real patient interactions.
%This finding suggests that the patient simulator is overall perceived as useful, but it may take experience with real patients to be able to provide a more nuanced assessment.

\paragraph{Perceived Skill Improvement}
Trainees also indicated that they believed \trainer{} would help improve their CBT formulation skills over both the GPT-4 baseline and their current training methods.
The trainees first compared \trainer with the baseline on a 5-point Likert scale, where higher scores indicate a higher degree of preference for \trainer. 
The trainees indicated that \trainer{} was better than the baseline at improving their CBT formulation skills (median: $4.0$, IQR: $3.5$-$4.5$).
Trainees also highlighted that \trainer{} was better at helping them improve their ability to identify beliefs (median: $3.5$, IQR: $2.5$-$4.5$) and maladaptive thinking (median: $4.0$, IQR: $3.0$-$4.5$).
Trainees then compared \trainer to their current training materials. 
Trainees indicated that \trainer was better at improving overall skills (median: $4.5$, IQR: $4.0$-$5.0$), as well as improving their ability to identify beliefs (median: $4.5$, IQR: $4.0$-$5.0$) and maladaptive thinking (median: $4.5$, IQR: $4.0$-$5.0$).
Taken together, these results indicate that not only does \trainer fill a perceived gap in the existing training methodology, but \trainer is preferred by trainees compared to a strong GPT-4 baseline for improving CBT formulation skills.

\paragraph{Perceived Confidence Improvement} 
In our formative study, both trainees and experts indicated that a simulated patient framework could help improve their confidence in interacting with real patients.
To evaluate this perceived confidence improvement, we first asked the trainees to compare \trainer{} and the baseline on a 5-point Likert scale, where higher scores indicate more preference for \trainer. 
All trainees indicated that \trainer would be ``much better'' for improving their confidence for real patient interactions (median: $5.0$, IQR: $4.5$-$5.0)$. 
We then asked trainees to compare \trainer with their formal CBT training in terms of its ability to improve their confidence in handling real patient interactions.
Again, the trainees strongly favored \trainer (median: $5.0$, IQR: $4.5$-$5.0$) over existing training methods.
These results indicate that practicing with \trainer can bring substantial perceived confidence improvements for CBT formulation compared to both a strong GPT-4 baseline and existing CBT training.
%One participant who had yet to work with real patients noted that \trainer{} could help build confidence due to its ability to check one's own responses.
%Another participant echoed this benefit, indicating that the ability to save and review interactions with the tool is invaluable for educational purposes, as instructors could review the transcripts to provide detailed and targeted feedback. 
%This ability is limited for in-person roleplays due to logistical constraints. 

\begin{comment}
\subsubsection{Feedback and Discussions}
We also asked the trainees to discuss the pros and cons of the tools. 
We highlight some of these results here.
One trainee highlighted that the general framework of simulated patient tools offered significant advantages, such as providing a more realistic experience compared to students role-playing patients, reducing awkwardness in peer interactions, and allowing for the saving and review of interactions for educational feedback. 
They also appreciated that the tool enables repetitive practice in a controlled environment, which could greatly aid skill development. 
However, this participant cautioned that the tool lacks the emotional depth and urgency of real patient interactions, which may limit its effectiveness in fully replicating the complexity of clinical training.
This feedback supports the need for even more customizable parameters in the tool to allow trainees to explore different challenges that they may face in their real clinical training.
\end{comment}

%\subsection{Automatic Evaluations}
%\zhiyu{Some GPT-4 or other auto results here.}
